Measurement of the thermal accommodation coefficient of helium on a crystalline silicon surface at low-temperatures

Next-generation gravitational wave observatories are expected to use cryogenically cooled, pendulum-suspended 200 kg test mass mirrors from a crystalline material such as crystalline silicon. During operation of the observatories, these mirrors undergo heating due to the absorption of laser radiation of up to a watt. Low noise cooling techniques need to be developed. Low-pressure helium exchange gas at 5 K might contribute to the challenging task. Here, we report the measurement of the helium accommodation coefficient $\alpha(11\,\mathrm{K}<T< 30\,\mathrm{K})$, which is the probability that a helium atom thermalises with a surface at a given temperature, when reflected from it. We find $\alpha(T) > 0.7$ for temperatures < 20 K, which increases the cooling power compared to recently used assumptions. The idea of free molecular flow helium gas cooling is thus supported and might find application in some observatory concepts.

==> content/version.tex <==
Draft from commit 
6bc9536
 compiled on \today at  \currenttime.

